Spline Regression with Automatic Knot Selection

In this paper we introduce a new method for automatically selecting knots in spline regression. The approach consists in setting a large number of initial knots and fitting the spline regression through a penalized likelihood procedure called adaptive ridge. The proposed method is similar to penalized spline regression methods (e.g. P-splines), with the noticeable difference that the output is a sparse spline regression with a small number of knots. We show that our method called A-spline, for adaptive splines yields sparse regression models with high interpretability, while having similar predictive performance similar to penalized spline regression methods. A-spline is applied both to simulated and real dataset. A fast and publicly available implementation in R is provided along with this paper.

==> bump_table.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Sun Jun  3 18:05:39 2018
\scalebox{0.8}{
\begin{tabular}{lrrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{3}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-4}
 \textbf{} & \textbf{A} & \textbf{P} & \textbf{Smooth}\\
 \midrule
50 & 0.03 & 0.01 & 0.01 \\ 
  100 & 0.00 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> bump_table_a.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 11:39:53 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.0623 & $\bm{0.0583}$ & 0.0671 \\ 
  100 & 0.0207 & 0.0115 & $\bm{0.0101}$ \\ 
  200 & 0.0087 & $\bm{0.0052}$ & 0.0054 \\ 
  400 & 0.0038 & $\bm{0.0026}$ & 0.0027 \\ 
   \hline
\end{tabular}


==> bump_table_crit_homo.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:26:34 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.02207 & $\bm{0.01921}$ & 0.02431 \\ 
  100 & 0.00776 & 0.00415 & $\bm{0.004}$ \\ 
  200 & 0.00323 & $\bm{0.00186}$ & 0.0019 \\ 
  400 & 0.00151 & $\bm{0.00091}$ & 0.00093 \\ 
   \hline
\end{tabular}


==> bump_table_hetero.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:27:17 2018
\scalebox{0.8}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.01 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> bump_table_homo.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:19:55 2018
\scalebox{0.75}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.01 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> homo_bump_table.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jun 11 08:51:33 2018
\scalebox{0.8}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.01 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> homo_logit_table.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jun 11 08:51:39 2018
\scalebox{0.8}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.00 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> homo_sine_table.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jun 11 08:51:43 2018
\scalebox{0.85}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.01 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> homo_spa_het_table.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jun 11 08:51:48 2018
\scalebox{0.85}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.00 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> logit_table.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Sun Jun  3 15:03:52 2018
\scalebox{0.8}{
\begin{tabular}{lrrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{3}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-4}
 \textbf{} & \textbf{A} & \textbf{P} & \textbf{Smooth}\\
 \midrule
50 & 0.02 & 0.00 & 0.00 \\ 
  100 & 0.00 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> logit_table_a.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 11:39:55 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.0638 & $\bm{0.0576}$ & 0.0684 \\ 
  100 & 0.0209 & 0.0082 & $\bm{0.0077}$ \\ 
  200 & 0.0071 & $\bm{0.0036}$ & 0.0044 \\ 
  400 & 0.0034 & $\bm{0.0017}$ & 0.0018 \\ 
   \hline
\end{tabular}


==> logit_table_crit_hetero.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:27:21 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.02011 & $\bm{0.01901}$ & 0.02061 \\ 
  100 & 0.00699 & 0.00541 & $\bm{0.00413}$ \\ 
  200 & 0.00339 & 0.00224 & $\bm{0.00176}$ \\ 
  400 & 0.00162 & 0.00093 & $\bm{0.00081}$ \\ 
   \hline
\end{tabular}


==> logit_table_hetero.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:27:17 2018
\scalebox{0.8}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.00 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> logit_table_homo.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:19:55 2018
\scalebox{0.75}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.00 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> sine3_table_a.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Sat Jun  2 22:47:45 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.0215 & $\bm{0.0194}$ & 0.0243 \\ 
  100 & 0.0077 & 0.0033 & $\bm{0.0025}$ \\ 
  200 & 0.0030 & 0.0013 & $\bm{0.0012}$ \\ 
  400 & 0.0013 & $\bm{7e-04}$ & 8e-04 \\ 
   \hline
\end{tabular}


==> sine_table.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Sun Jun  3 15:03:52 2018
\scalebox{0.85}{
\begin{tabular}{lrrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{3}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-4}
 \textbf{} & \textbf{A} & \textbf{P} & \textbf{Smooth}\\
 \midrule
50 & 0.02 & 0.01 & 0.01 \\ 
  100 & 0.00 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> sine_table_a.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 11:39:56 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.0649 & $\bm{0.0601}$ & 0.0651 \\ 
  100 & 0.0207 & 0.0115 & $\bm{0.0107}$ \\ 
  200 & 0.0084 & $\bm{0.0057}$ & 0.006 \\ 
  400 & 0.0041 & $\bm{0.003}$ & 0.0033 \\ 
   \hline
\end{tabular}


==> sine_table_crit_hetero.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:27:21 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.02015 & $\bm{0.01891}$ & 0.02143 \\ 
  100 & 0.00748 & 0.00572 & $\bm{0.00524}$ \\ 
  200 & 0.00353 & 0.00268 & $\bm{0.00265}$ \\ 
  400 & 0.00172 & $\bm{0.00135}$ & 0.00144 \\ 
   \hline
\end{tabular}


==> sine_table_hetero.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:27:17 2018
\scalebox{0.85}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.01 \\ 
  100 & 0.01 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> sine_table_homo.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:19:56 2018
\scalebox{0.75}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.01 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> spa_het_table.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Sun Jun  3 15:03:52 2018
\scalebox{0.85}{
\begin{tabular}{lrrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{3}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-4}
 \textbf{} & \textbf{A} & \textbf{P} & \textbf{Smooth}\\
 \midrule
50 & 0.02 & 0.00 & 0.00 \\ 
  100 & 0.00 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> spa_het_table_a.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 11:39:56 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.0623 & $\bm{0.0581}$ & 0.0672 \\ 
  100 & 0.0200 & 0.0083 & $\bm{0.0062}$ \\ 
  200 & 0.0075 & $\bm{0.0034}$ & 0.0035 \\ 
  400 & 0.0034 & $\bm{0.0019}$ & 0.0019 \\ 
   \hline
\end{tabular}


==> spa_het_table_crit_homo.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:26:35 2018
\begin{tabular}{llll}
  \hline
Sample size & AIC & BIC & EBIC \\ 
  \hline
50 & 0.02109 & $\bm{0.01916}$ & 0.02401 \\ 
  100 & 0.00760 & 0.00305 & $\bm{0.00267}$ \\ 
  200 & 0.00292 & $\bm{0.00145}$ & 0.00152 \\ 
  400 & 0.00136 & $\bm{0.00078}$ & 8e-04 \\ 
   \hline
\end{tabular}


==> spa_het_table_hetero.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:27:17 2018
\scalebox{0.85}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.00 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}


==> spa_het_table_homo.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Jul 16 13:19:56 2018
\scalebox{0.75}{
\begin{tabular}{lrr}
  \toprule
  \multicolumn{1}{c}{\textbf{Sample size}} & \multicolumn{2}{c}{\textbf{Spline Regression Method}}\\
 \cmidrule(lr){2-3}
 \textbf{} & \textbf{A} & \textbf{P}\\
 \midrule
50 & 0.02 & 0.00 \\ 
  100 & 0.00 & 0.00 \\ 
  200 & 0.00 & 0.00 \\ 
  400 & 0.00 & 0.00 \\ 
   \bottomrule
\end{tabular}
}

